Transformer Multivariate Forecasting: Less is More?

In the domain of multivariate forecasting, transformer models stand out as powerful apparatus, displaying exceptional capabilities in handling messy datasets from real-world contexts. However, the inherent complexity of these datasets, characterized by numerous variables and lengthy temporal sequences, poses challenges, including increased noise and extended model runtime. This paper focuses on reducing redundant information to elevate forecasting accuracy while optimizing runtime efficiency. We propose a novel transformer forecasting framework enhanced by Principal Component Analysis (PCA) to tackle this challenge. The framework is evaluated by five state-of-the-art (SOTA) models and four diverse real-world datasets. Our experimental results demonstrate the framework's ability to minimize prediction errors across all models and datasets while significantly reducing runtime. From the model perspective, one of the PCA-enhanced models: PCA+Crossformer, reduces mean square errors (MSE) by 33.3% and decreases runtime by 49.2% on average. From the dataset perspective, the framework delivers 14.3% MSE and 76.6% runtime reduction on Electricity datasets, as well as 4.8% MSE and 86.9% runtime reduction on Traffic datasets. This study aims to advance various SOTA models and enhance transformer-based time series forecasting for intricate data. Code is available at: https://github.com/jingjing-unilu/PCA_Transformer.

==> Methodology.tex <==
\section{Methodology}
\label{methodology}
\subsection{Problem Formulation}
We aim to solve the following problem: given past observations of time series $ H = (x^{1}, x^{2}, ..., x^{M}, y)\in \mathbb{R}^{T\times (M+1)} $ where the M represents different variables, the $y$ denotes targets and the $T$ is the length of time series. The $m$-th variable is denoted as $x^{m} = (x_{1}^{m}, x_{2}^{m}, ..., x_{T}^{m})^\top\in \mathbb{R}^{T}$. The target can be denoted as $y = (y_{1}, y_{2}, ..., y_{T})^\top\in \mathbb{R}^{T}$. We aim to forecast $F$ future values of the target $(y_{T+1}, y_{T+2}, ..., y_{T+F})^\top$.

\subsection{Structure Overview}
The schematic representation of our framework is illustrated in Figure \ref{structure_overview}, with the Transformer serving as the backbone architecture. To initiate the process, we load the original data, encompassing all pertinent variables. Subsequently, Principal Components Analysis (PCA) is applied to all variables, facilitating a reduction in dimensionality from $M$ to $P$ variables. The target data is deliberately excluded from this process to prevent information leakage. Following this, the dataset undergoes partitioning into training and testing subsets (validation subset will be included based on models) for model evaluation. The pre-processed dataset is then seamlessly fed into the Transformer-based forecasting model. Finally, the forecasting model generates $F$ future predicted values for the target.

\subsubsection{PCA Process.}
In the PCA process, we utilize the randomized singular value decomposition (SVD) based PCA~\cite{scikit-learn,halko2011finding,szlam2014implementation} due to our large dataset. The input data of the PCA process is $ H_{T\times M} = (x^{1}, x^{2}, ..., x^{M})\in \mathbb{R}^{T\times M} $. The output data is $ H_{T\times P}' = (x^{1}, x^{2}, ..., x^{P})\in \mathbb{R}^{T\times P} $. $P$ is the components numbers of the PCA.
The calculation steps are shown as follows:
\begin{enumerate}
\item Center the dataset. For each variable $x^{m}$ in the input data $H_{T\times M}$, we center the data such as $\tilde{x^{m}} = (x_{1}^{m}-\bar{x^{m}}, x_{2}^{m}-\bar{x^{m}}, ..., x_{T}^{m}-\bar{x^{m}})^\top$, where $\bar{x^{m}}=\frac{1}{T}\sum x^{m}$. Then we obtain centered data: $\tilde{H_{T\times M}} = $ $(\tilde{x^{1}}, \tilde{x^{2}}, ..., \tilde{x^{M}})$
\item Calculate the covariance matrix for  $\tilde{H_{T\times M}}$, then we get the $\tilde{CH_{T\times M}}$
\item Apply SVD: 1) $\tilde{CH_{T\times M}} \approx U_{T\times T}\Sigma_{T \times M} (V_{M \times M})^\top $\\
2) $\tilde{H_{T\times M}}' = \tilde{CH_{T\times M}} \times V_{M \times M} \approx U_{T\times T}\Sigma_{T\times M}$
\item  Get $top$-$P$ principal components. $\Sigma_{T\times M}$ is the singular values of $\tilde{CH_{T\times M}}$ and its elements (non-zero singular values) are the rank of $\tilde{CH_{T\times M}}$. Thus, we get $top$-$P$ principal components according to the rank. So the $P$ principal components of the input data $H_{T\times M}$ is $\tilde{H_{T\times P}}' = U_{T\times T}\Sigma_{T\times P}$.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Transformer-based Time Series Forecasting Models.}
Transformer-based Time series forecasting models adhere to the classic transformer components and architecture, as depicted in Figure \ref{Tran_arch}. transformer-based forecasting models can be divided into 4 categories as show in Table \ref{tran_cate}. In this paper, we use the typical models in each category like Informer, Autoformer, Crossformer, Non-stationary Transformer, PatchTST, iTransfromer. 





==> app.tex <==
% \newpage
\appendix
\section{Appendix}
The following contents are all Appendix. 
\subsubsection{Get Table~\ref{impro_result_PCA_tran} from Table~\ref{acc_result_PCA_tran} and Table~\ref{result_ela_time}.} Table~\ref{impro_result_PCA_tran} serves as a consolidation of accuracy results from Table~\ref{acc_result_PCA_tran} and corresponding runtime results from Table~\ref{result_ela_time}. Each entry in Table~\ref{impro_result_PCA_tran} represents the best-performing (lowest MSE, bold with blue cell color) model from Table~\ref{acc_result_PCA_tran}, along with its associated runtime, in comparison with the original (w/o PCA) model and its corresponding time. For instance, the optimal performance of PCA+PatchTST on the Electricity dataset in Table~\ref{acc_result_PCA_tran} is 0.30114 (lowest MSE, bold with blue cell color), compared to 0.60771 (w/o PCA). Consequently, the reduction in MSE for PCA+PatchTST on the electricity dataset is 2.14\%, as reflected in Table~\ref{impro_result_PCA_tran}.
% %%%%%%%%%%%%%%%%%
% \begin{table*}[!ht]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|c|c|rr|rr|rr|rr|rr|rr}
% \toprule
% \multirow{2}{*}{\textbf{Dataset}}                       & \textbf{Variables}       & \textbf{PCA} & \multicolumn{2}{c|}{\textbf{PCA+PatchTST}}                             & \multicolumn{2}{c|}{\textbf{PCA+Crossformer}}                          & \multicolumn{2}{c|}{\textbf{PCA+Autoformer}}                           & \multicolumn{2}{c|}{\textbf{PCA+N.S. Trans.}}           & \multicolumn{2}{c|}{\textbf{PCA+iTransformer}}         & \multicolumn{2}{c}{\textbf{PCA+Transformer}}                          \\ 
%  & \textbf{w/o Target}       & \textbf{Components} & \multicolumn{2}{c|}{(\bf MSE $\mid$ \bf MAE)}    & \multicolumn{2}{c|}{(\bf MSE $\mid$ \bf MAE)}  & \multicolumn{2}{c|}{(\bf MSE $\mid$ \bf MAE)}   & \multicolumn{2}{c|}{(\bf MSE $\mid$ \bf MAE)}       & \multicolumn{2}{c|}{(\bf MSE $\mid$ \bf MAE)}  & \multicolumn{2}{c}{(\bf MSE $\mid$ \bf MAE)}        
%  \\ 
% \midrule
%      &                                & \textbf{2}              & \cellcolor[HTML]{D4E6F1}{\bf 0.05561}   & 0.17868       & 0.19371 & 0.38307      & \cellcolor[HTML]{D4E6F1}{\bf 0.08919} & \bf 0.22736   
%      & \cellcolor[HTML]{D4E6F1}{\bf 0.07144}   & \bf 0.20484       & 0.05736 & 0.18378                    & 0.85307  & 0.88175               \\ 
% % %%\cline{3-15} 
%      &                                & \textbf{4}              & {0.05671} & 0.18052                     & {\cellcolor[HTML]{D4E6F1}{\bf 0.16091}}  & {\bf 0.33508}         & {0.10550} & 0.25530                          & {0.08048} & 0.21217               & {\cellcolor[HTML]{D4E6F1}{\bf 0.05637}}   & {\bf 0.18241}                      & {1.17205} & 1.01673               \\ 
% %\cline{3-15} 
% \multirow{-3}{*}{\textbf{ETTh1}}        & \multirow{-3}{*}{\textbf{6}}   & \textbf{w/o PCA}        & {0.05575} & {\bf 0.17838}        & {0.36994} & 0.55491               & {0.11395}   & 0.25875               & {0.07814}  & 0.21079               & {0.05662} & 0.18278                  & {\cellcolor[HTML]{D4E6F1}{\bf 0.72492}}   & {\bf 0.79393}  
% \\ 
% \midrule
%      &                                & \textbf{2}              & {0.0013408}  & 0.0267667         & {0.0066745}  & 0.0669198                                & {0.0390251} & 0.0985756                         & {\cellcolor[HTML]{D4E6F1}{\bf 0.0012783}} & {\bf 0.0262055}           & {\cellcolor[HTML]{D4E6F1}{\bf 0.0012391}} & {\bf 0.0258336}                    & {0.0074935} & 0.0697642    
% \\ 
% % %%\cline{3-15} 
%      &                                & \textbf{5}              & {0.0013426} & 0.0266463            & {0.0039031}  & 0.0495619                                & {0.0086512}  & 0.0701804             & {0.0013453} & 0.0270548             & {0.0012655} & 0.0262108                       & {0.0031227}  & 0.0433567                   
% \\ 
% % %%\cline{3-15} 
%      &                                & \textbf{10}             & {0.0013277}  & 0.0265256             & {0.0044438} & 0.0535568                           & {0.0114851} & 0.0851401             & {0.0015487}  & 0.0288031             & {0.0012676} & 0.0260793       & {0.0051427}  & 0.0554222        
% \\
% % %%\cline{3-15} 
%      &                                & \textbf{15}             & {0.0013124}  & 0.0266787            & {\cellcolor[HTML]{D4E6F1}{\bf 0.0019383}} & {\bf 0.0324117}                      & {\cellcolor[HTML]{D4E6F1}{\bf 0.0072318}} & {\bf 0.0679583}                       & {0.0018783} & 0.0313342             & {0.0013160}  & 0.0265606                                & {0.0040705}  & 0.0517972                     
% \\ 
% %\cline{3-15} 
% \multirow{-5}{*}{\textbf{Weather}} & \multirow{-5}{*}{\textbf{20}}  & \textbf{w/o PCA}        & {\cellcolor[HTML]{D4E6F1}{\bf 0.0013116}} & {\bf 0.0263536}           & {0.0045753}& 0.0548066                     & {0.0079332}  & 0.0704268             & {0.0016366} & 0.0294900             & {0.0013511}  & 0.0271509                                 & {\cellcolor[HTML]{D4E6F1}{\bf 0.0025455}} & {\bf 0.0372824} 
% \\ 
% \midrule
%      &                                & \textbf{2}              & {\cellcolor[HTML]{D4E6F1}{\bf 0.30114}}   & {\bf 0.39454}        & {0.24117} & 0.35286                        & {0.41615} & 0.49454                       & {0.32548} & 0.42185               & {0.35119} & 0.43913& {\cellcolor[HTML]{D4E6F1}{\bf 0.31722}}   & {\bf 0.42333}   
% \\ 
% % %%\cline{3-15} 
%      &                                & \textbf{20}             & {0.30803}  & 0.40253          & {0.31382} & 0.39153                         & {0.39585}  & 0.47261                     & {0.35360} & 0.44082            & {0.31114} & 0.41341                                  & {0.44774}   & 0.50390         
% \\ 
% % %%\cline{3-15} 
%      &                                & \textbf{40}             & {0.31029}  & 0.40227               & {0.32395}  & 0.39478                     & {0.38023}  & 0.46607                    & {0.38404} & 0.44949               & {0.34803}  & 0.43267                        & {0.45457}  & 0.49402             
% \\ 
% %%\cline{3-15} 
%      &                                & \textbf{80}             & {0.30792}  & 0.40005           & {\cellcolor[HTML]{D4E6F1}{\bf 0.23528}}   & {\bf 0.34291}         & {0.42425} & 0.48486& {0.31263} & 0.41109             & {0.28967} & 0.39682                                  & {0.36052} & 0.44804               
% \\ 
% %%\cline{3-15} 
%      &                                & \textbf{160}            & {0.30951} & 0.39863   & {0.30753}& 0.38397                       & {0.38894}  & 0.47346                                 & {0.32938}  & 0.42110               & {0.31660} & 0.41921                         & {0.48044}   & 0.51270     
% \\ 
% %%\cline{3-15} 
%      &                                & \textbf{240}            & {0.31747}   & {0.40354}                             & {0.26574}  & {0.36454}                        & {0.42832} & {0.49689}                               & {0.34589}  & {0.43446}                             & {\cellcolor[HTML]{D4E6F1}{\bf 0.25611}}   & {\bf 0.36751}         & {0.37116} & {0.45557}                             
% \\ 
% %\cline{3-15} 
% \multirow{-7}{*}{\textbf{Electricity}}  & \multirow{-7}{*}{\textbf{320}} & \textbf{w/o PCA}        & {0.30771} & 0.40156             & {0.27444}  & 0.36760                   & \cellcolor[HTML]{D4E6F1}{\bf 0.37565}  & {\bf 0.46435}                              & \cellcolor[HTML]{D4E6F1}{\bf 0.30231}  & {\bf 0.40977}              & {0.54722}  & 0.54924                                 & {0.39571} & 0.46279      
% \\ 
% \midrule
%      &                                & \textbf{1}              & {0.17485}  & 0.25452        & \cellcolor[HTML]{D4E6F1}{\bf 0.14789} & {\bf 0.22577}                & {0.31848}  & 0.41374                                & {0.18998}   & {0.29156}                & {0.32595}  & 0.40816               & {0.28672}  & {0.35876}   
% \\ 
%      &                                & \textbf{2}              & {0.17714}  & 0.25728         & {0.16042} & 0.24255                & {0.29514}  & 0.39557                                & {\cellcolor[HTML]{D4E6F1}{\bf 0.17894}}   & {\bf 0.28501}                & {1.86223}  & 1.17306               & {\cellcolor[HTML]{D4E6F1}{\bf 0.28144}}   & {\bf 0.35329}   
% \\ 
% %%\cline{3-15} 
%      &                                & \textbf{25}             & {\cellcolor[HTML]{D4E6F1}{\bf 0.16754}}   & 0.24795                    & {0.25004}  & 0.31726         & {0.27335} & 0.36999                               & {0.22374}  & 0.33921               & {1.31162} & 0.93039                          & {0.29579} & 0.37345                  
% \\ 
% %%\cline{3-15} 
%      &                                & \textbf{50}             & {0.16907}  & 0.24932                     & {0.20874}   & 0.28413            & {\cellcolor[HTML]{D4E6F1}{\bf 0.24967}}   & {\bf 0.34481}   & {0.20833}  & 0.31271                             & {1.86220} & 1.17306                                  & {0.41403} & 0.43881  
% \\ 
% %%\cline{3-15} 
%      &                                & \textbf{105}            & {0.17121} & 0.25329                        & {0.23546} & 0.29953               & {0.30357}   & 0.40072                  & {0.19733}  & 0.30020               & {1.86222}  & 1.17307                     & {0.33498}  & 0.40060        
% \\
% %%\cline{3-15} 
%      &                                & \textbf{215}            & {0.17100}  & 0.24890                       & {0.16648} & 0.23886               & {0.37778}   & 0.44868                    & {0.23479}   & 0.33047               & {1.86224} & 1.17306                        & {0.35731}  & 0.41112       
% \\ 
% %%\cline{3-15} 
%      &                                & \textbf{430}            & {0.17507}  & 0.25062& {0.17663}   & 0.25027                              & {0.29786}   & 0.40188               & {0.27937} & 0.38314               & {1.86222} & 1.17307             & {0.38011}  & 0.41905   
% \\ 
% %%\cline{3-15} 
%      &                                & \textbf{645}            & {0.17123}   & 0.24950                                  & {0.21702}  & 0.28981                            & {0.31110} & 0.39311               & {0.37402}    & 0.45356               & {1.25570}   & 0.92052              & {0.33137}  & 0.39332                         
% \\ 
% %\cline{3-15} 
% \multirow{-9}{*}{\textbf{Traffic}}      & \multirow{-8}{*}{\textbf{861}} & \textbf{w/o PCA}        & {0.16831} & {\bf 0.24585}   & {{0.15540}}   & {0.22792}        & {0.30356}   & 0.40767               & {0.21742}  & 0.32678                                & {\cellcolor[HTML]{D4E6F1}{\bf 0.25060}}   & {\bf 0.35071}                      & {0.29690} & 0.35520                              
% \\ 
% \bottomrule
% \end{tabular}
% }
% \caption{Accuracy result of PCA-enhanced transformer forecasting models (PCA+N.S. Trans.: PCA + Non-stationary Transformer).}
% \label{acc_result_PCA_tran}
% \end{table*}
% %%%%
%%%%
% \begin{table*}[ht]
% \centering
% \resizebox{0.85\textwidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \toprule
% \multirow{2}{*}{\textbf{Dataset}}   & \textbf{Variables}  & \textbf{PCA} & {\textbf{PCA+}}  & {\textbf{PCA+}}  & {\textbf{PCA+}}    & {\textbf{PCA+N.S.}}    & {\textbf{PCA+}}   & {\textbf{PCA+}}   \\ 
% ~ & \textbf{w/o Target}       & \textbf{Components} & {\textbf{PatchTST}}     & {\textbf{Crossformer}}  & {\textbf{Autoformer}}   & {\textbf{Transformer}}     & {\textbf{iTransformer}} & {\textbf{Transformer}}   
%  \\ 
% \midrule
%      &                                & \textbf{2}              & {\cellcolor[HTML]{DDEBF7}\textbf{71}}                  & {241}               & \cellcolor[HTML]{DDEBF7}\textbf{310}                        & \cellcolor[HTML]{DDEBF7}\textbf{118}                          & 87  & 219 \\ 
     
%      &                                & \textbf{4}              & {64}                & {\cellcolor[HTML]{DDEBF7}\textbf{246}}                 & 311                      & 141                        & \cellcolor[HTML]{DDEBF7}\textbf{84}    & 126 \\ 
% \multirow{-3}{*}{\textbf{ETTh1}}        & \multirow{-3}{*}{\textbf{6}}   & \textbf{w/o PCA}        & {74}                & {252}               & {310} & {177}   & 88  & {\cellcolor[HTML]{DDEBF7}\textbf{126}}                 \\ \midrule
%      &                                & \textbf{2}              & 231 & 1915& 686                      & \cellcolor[HTML]{DDEBF7}\textbf{415}                          & \cellcolor[HTML]{DDEBF7}\textbf{653}   & 375 \\ 
%      &                                & \textbf{5}              & 241 & 1264& 690                      & 414                        & 538 & 377 \\ 
%      &                                & \textbf{10}             & 250 & 1399& 701                      & 416                        & 603 & 379 \\ 
%      &                                & \textbf{15}             & 283 & \cellcolor[HTML]{DDEBF7}\textbf{1224}  & \cellcolor[HTML]{DDEBF7}\textbf{689}                        & 418                        & 440 & 378 \\ 
% \multirow{-5}{*}{\textbf{Weather}} & \multirow{-5}{*}{\textbf{20}}  & \textbf{w/o PCA}        & \cellcolor[HTML]{DDEBF7}\textbf{311}   & 1768& {685} & {417}   & 625 & {\cellcolor[HTML]{DDEBF7}\textbf{378}}                 \\ \midrule
%      &                                & \textbf{2}              & \cellcolor[HTML]{DDEBF7}\textbf{221}   & { 1430}                                 & 975                      & 876                        & {200}                                  & \cellcolor[HTML]{DDEBF7}{\textbf{283}} \\ 
%      &                                & \textbf{20}             & 246 & {883}                                  & 723                      & 1198                       & {209}                                  & {241}                                  \\ 
%      &                                & \textbf{40}             & 352 & {904}                                  & 604                      & 1043                       & {207}                                  & {241}                                  \\ 
%      &                                & \textbf{80}             & 579 & {\cellcolor[HTML]{DDEBF7} \textbf{925}} & 733                      & 887                        & { 205}                                  & {245}                                  \\ 
%      &                                & \textbf{160}            & 1038& {1620}                                 & 748                      & 1394                       & { 216}                                  & {250}                                  \\ 
%      &                                & \textbf{240}            & 1510& { 2847}                                 & 622                      & 1418                       & \cellcolor[HTML]{DDEBF7}{\textbf{380}} & {303}                                  \\ 
% \multirow{-7}{*}{\textbf{Electricity}}  & \multirow{-7}{*}{\textbf{320}} & \textbf{w/o PCA}        & 1953              & 3960            & \cellcolor[HTML]{DDEBF7}\textbf{759}                        & \cellcolor[HTML]{DDEBF7}\textbf{1768}                         & {287}                                  & {303}                                  
% \\ 
% \midrule
%      &                                & \textbf{1}              & 667 & \cellcolor[HTML]{DDEBF7}\textbf{2590} & 320                      & {{146}}     & 346 & {{135}} 
%      \\ 
%      &                                & \textbf{2}              & 735 & 2672& 322                      & {\cellcolor[HTML]{DDEBF7}\textbf{149}}     & 378 & {\cellcolor[HTML]{DDEBF7} \textbf{136}} 
%      \\ 
%      &                                & \textbf{25}             &{\cellcolor[HTML]{DDEBF7} \textbf{716}} & 2395& 321                      & 152                        & 162 & 138 \\ 
%      &                                & \textbf{50}             & 726 & 2670& {\cellcolor[HTML]{DDEBF7}{\textbf{330}}} & {153} & 329 & 139 \\ 
%      &                                & \textbf{105}            & 743 & 2760& 330                      & 155                        & 358 & 141 \\ 
%      &                                & \textbf{215}            & 1285& 6122& 332                      & 159                        & 409 & 145 \\ 
%      &                                & \textbf{430}            & 2398& 10330                                  & 348                      & 167                        & 683 & 154 \\ 
%      &                                & \textbf{645}            & 3554& 10171                                  & 353                      & 177                        & 755 & 162 \\ 
% \multirow{-9}{*}{\textbf{Traffic}}      & \multirow{-8}{*}{\textbf{861}} & \textbf{w/o PCA}        & 4626& {{19749}}               & 354                      & 173                        & \cellcolor[HTML]{DDEBF7}\textbf{625}   & 154 \\ 
% \midrule
% \end{tabular}
% }
% \caption{Runtime result of PCA-enhanced transformers forecasting model (unit: second).}
% \label{result_ela_time}
% \end{table*}
